Sign-switchable and tunable macroscopic curvature of liquid jets by microscopic laser-induced cavitation

Localized forcing of liquid jets can trigger Rayleigh-Plateau breakup at low perturbation amplitudes or explosive fragmentation at high amplitudes, while controlled bending in the intermediate regime has remained unexplored. We show that femtosecond-laser-induced cavitation, seeded at the interface of a 100 micrometre-diameter water jet, produces a selectable curvature in 0.4-1 mm long segments. Cavitation rupturing at the liquid-air interface drives fast outward jetting and induces a slower recoil on the opposite boundary, which evolves on the capillary-inertial timescale and results in curving of the liquid segment. The curvature is governed by three laser parameters. Off-axis laser illumination on the jet shifts the refractive caustics and redistributes energy deposition between the front and rear interfaces. The resulting recoil imbalance determines the curvature sign, with a straight configuration in the balanced case. Laser energy offers additional control over the recoil impulse via plasma defocusing and nonlinear absorption in the liquid jet, where the response is bounded by axisymmetric deformation at low energy and explosive vaporization at high energy. Repetition rate sets the spacing between successive cavitation events and hence the length of the bent segment. Curvature extends across the segment for lengths of 6-10 jet diameters; shorter segments undergo Rayleigh-Plateau breakup, whereas longer ones bend mainly near their retracting ends. Our results offer a platform for optofluidic control of switchable and tunable macroscopic curvature in flowing liquid jets.

==> ref.tex <==
@article{Zhang1988,
  title   = {Shape distortion of a single water droplet by laser-induced electrostriction},
  author  = {Zhang, J. and Chang, R. K.},
  journal = {Optics Letters},
  volume  = {13},
  number  = {10},
  pages   = {916--918},
  year    = {1988},
  doi     = {10.1364/OL.13.000916},
}

@article{Klein2015,
  title   = {Drop Shaping by Laser-Pulse Impact},
  author  = {Klein, A. L. and Bouwhuis, W. and Visser, C. W. and Lhuissier, H. and Sun, C. and Snoeijer, J. H. and Villermaux, E. and Lohse, D. and Gelderblom, H.},
  journal = {Physical Review Applied},
  volume  = {3},
  pages   = {044018},
  year    = {2015},
  doi     = {10.1103/PhysRevApplied.3.044018},
}

@article{Cheng2025,
  title   = {Particulate reshapes surface jet dynamics induced by a cavitation bubble},
  author  = {Cheng, Xianggang and Chen, Xiao-Peng and Yuan, Zhi-Ming and Jia, Laibing},
  journal = {Nature Communications},
  volume  = {16},
  pages   = {7562},
  year    = {2025},
  doi     = {10.1038/s41467-025-62936-y},
}

@article{Patrascioiu2014,
  title   = {Laser-generated liquid microjets: correlation between bubble dynamics and liquid ejection},
  author  = {Patrascioiu, A. and Fern{\'a}ndez-Pradas, J. M. and Palla-Papavlu, A. and others},
  journal = {Microfluidics and Nanofluidics},
  volume  = {16},
  pages   = {55--63},
  year    = {2014},
  doi     = {10.1007/s10404-013-1220-4},
}

@article{Nakagawa2017,
  title   = {Pulsed laser-induced liquid jet: evolution from shock/bubble interaction to neurosurgical application},
  author  = {Nakagawa, A. and Kumabe, T. and Ogawa, Y. and others},
  journal = {Shock Waves},
  volume  = {27},
  pages   = {1--14},
  year    = {2017},
  doi     = {10.1007/s00193-016-0660-6},
}

@article{Sonden1996,
  title   = {Laser-induced shock wave endothelial cell injury},
  author  = {Sond{\'e}n, A. and Svensson, B. and Roman, N. and Ostmark, H. and Brismar, B. and Palmblad, J. and Kjellstr{\"o}m, B. T.},
  journal = {Lasers in Surgery and Medicine},
  volume  = {26},
  number  = {4},
  pages   = {364--375},
  year    = {2000},
  doi     = {10.1002/(SICI)1096-9101(2000)26:4<364::AID-LSM4>3.0.CO;2-3},
}

@article{Li2018,
  title   = {Counter-jet formation of an expanding bubble near a curved elastic boundary},
  author  = {Li, S. and Zhang, A.-M. and Han, R.},
  journal = {Physics of Fluids},
  volume  = {30},
  pages   = {121703},
  year    = {2018},
  doi     = {10.1063/1.5063835},
}

@article{Supponen2015,
  title   = {Detailed jet dynamics in a collapsing bubble},
  author  = {Supponen, O. and Obreschkow, D. and Kobel, P. and Farhat, M.},
  journal = {Journal of Physics: Conference Series},
  volume  = {656},
  pages   = {012038},
  year    = {2015},
  doi     = {10.1088/1742-6596/656/1/012038},
}

@article{Kohsakowski2017,
  title   = {High productive and continuous nanoparticle fabrication by laser ablation of a wire-target in a liquid jet},
  author  = {Kohsakowski, S. and Santagata, A. and Dell'Aglio, M. and de Giacomo, A. and Barcikowski, S. and Wagener, P. and G{\"o}kce, B.},
  journal = {Applied Surface Science},
  volume  = {418},
  pages   = {86--92},
  year    = {2017},
  doi     = {10.1016/j.apsusc.2017.02.174},
}

@article{Reuter2017,
  title   = {Cavitation erosion by shockwave self-focusing of a single bubble},
  author  = {Reuter, F. and Deiter, C. and Ohl, C.-D.},
  journal = {Ultrasonics Sonochemistry},
  volume  = {37},
  pages   = {542--549},
  year    = {2017},
  doi     = {10.1016/j.ultsonch.2017.02.004},
}

@article{Han2019,
  title   = {Interaction of cavitation bubbles with the interface of two immiscible fluids on multiple time scales},
  author  = {Han, R. and Zhang, A.-M. and Tan, S. and Li, S.},
  journal = {Journal of Fluid Mechanics},
  volume  = {883},
  pages   = {A36},
  year    = {2019},
  doi     = {10.1017/jfm.2019.898},
}

@article{Sun2009,
  title   = {Growth and collapse of a vapour bubble in a microtube: The role of thermal effects},
  author  = {Sun, C. and Can, E. and Dijkink, R. and Lohse, D. and Prosperetti, A.},
  journal = {Journal of Fluid Mechanics},
  volume  = {632},
  pages   = {5},
  year    = {2009},
  doi     = {10.1017/S0022112009007381},
}

@article{Tagawa2012,
  title   = {Highly focused supersonic microjets},
  author  = {Tagawa, Y. and Oudalov, N. and Visser, C. W. and Peters, I. R. and van der Meer, D. and Sun, C. and Prosperetti, A. and Lohse, D.},
  journal = {Physical Review X},
  volume  = {2},
  pages   = {031002},
  year    = {2012},
  doi     = {10.1103/PhysRevX.2.031002},
}

@article{Vogel2005,
  title   = {Mechanisms of femtosecond laser nanosurgery of cells and tissues},
  author  = {Vogel, A. and Noack, J. and H{\"u}ttman, G. and Paltauf, G.},
  journal = {Applied Physics B},
  volume  = {81},
  pages   = {1015--1047},
  year    = {2005},
  doi     = {10.1007/s00340-005-2036-6},
}

@article{Linz2025,
  title   = {Laser-induced plasma formation and cavitation in water: from nanoeffects to extreme states of matter},
  author  = {Linz, Norbert and Freidank, Sebastian and Liang, Xiao-Xuan and Vogel, Alfred},
  journal = {Reports on Progress in Physics},
  volume  = {88},
  pages   = {088501},
  year    = {2025},
  doi     = {10.1088/1361-6633/adedb3},
}

@book{Chin2010,
  title     = {Femtosecond Laser--Matter Interaction},
  editor    = {Chin, S. L.},
  publisher = {Springer},
  address   = {Berlin},
  year      = {2010},
}

@article{Perry1994,
  title   = {Terawatt to petawatt subpicosecond lasers},
  author  = {Perry, M. D. and Mourou, G.},
  journal = {Science},
  volume  = {264},
  pages   = {917--924},
  year    = {1994},
  doi     = {10.1126/science.264.5161.917},
}

@article{Chichkov1996,
  title   = {Femtosecond, picosecond and nanosecond laser ablation of solids},
  author  = {Chichkov, B. N. and Momma, C. and Nolte, S. and von Alvensleben, F. and T{\"u}nnermann, A.},
  journal = {Applied Physics A},
  volume  = {63},
  pages   = {109--115},
  year    = {1996},
  doi     = {10.1007/BF01567637},
}

@article{Nolte1997,
  title   = {Ablation of metals by ultrashort laser pulses},
  author  = {Nolte, S. and Will, M. and Burghoff, J. and T{\"u}nnermann, A.},
  journal = {Journal of the Optical Society of America B},
  volume  = {14},
  pages   = {2716--2722},
  year    = {1997},
  doi     = {10.1364/JOSAB.14.002716},
}

@article{Gattass2008,
  title   = {Femtosecond laser micromachining in transparent materials},
  author  = {Gattass, R. R. and Mazur, E.},
  journal = {Nature Photonics},
  volume  = {2},
  pages   = {219--225},
  year    = {2008},
  doi     = {10.1038/nphoton.2008.47},
}

@article{Vogel2003,
  title   = {Mechanisms of pulsed laser ablation of biological tissues},
  author  = {Vogel, A. and Venugopalan, V.},
  journal = {Chemical Reviews},
  volume  = {103},
  pages   = {577},
  year    = {2003},
  doi     = {10.1021/cr010379n},
}

@article{Rossello2022,
  title   = {Dynamics of pulsed laser-induced cavities on a liquid--gas interface: from a conical splash to a bullet jet},
  author  = {Rossell{\'o}, J. M. and Reese, H. and Ohl, C.-D.},
  journal = {Journal of Fluid Mechanics},
  volume  = {939},
  pages   = {A35},
  year    = {2022},
  doi     = {10.1017/jfm.2022.223},
}

@article{Rossello2023,
  title   = {Bubble nucleation and jetting inside a millimetric droplet},
  author  = {Rossell{\'o}, J. M. and Reese, H. and Raman, K. A. and Ohl, C.-D.},
  journal = {Journal of Fluid Mechanics},
  volume  = {968},
  pages   = {A19},
  year    = {2023},
  doi     = {10.1017/jfm.2023.516},
}

@article{Krivokorytov2018,
  title   = {Shaping and controlled fragmentation of liquid metal droplets through cavitation},
  author  = {Krivokorytov, M. S. and others},
  journal = {Scientific Reports},
  volume  = {8},
  pages   = {597},
  year    = {2018},
  doi     = {10.1038/s41598-017-19110-9},
}

@article{Saurel2008,
  title   = {Modelling phase transition in metastable liquids: application to cavitating and flashing flows},
  author  = {Saurel, R. and Petitpas, F. and Abgrall, R.},
  journal = {Journal of Fluid Mechanics},
  volume  = {607},
  pages   = {313--350},
  year    = {2008},
  doi     = {10.1017/S0022112008002061},
}

@article{Gonzalez2016,
  title   = {Fragmentation of acoustically levitating droplets by laser-induced cavitation bubbles},
  author  = {Gonzalez Avila, S. R. and Ohl, C.-D.},
  journal = {Journal of Fluid Mechanics},
  volume  = {805},
  pages   = {551--576},
  year    = {2016},
  doi     = {10.1017/jfm.2016.583},
}

@article{Benjamin1966,
  title   = {The collapse of cavitation bubbles and the pressures thereby produced against solid boundaries},
  author  = {Benjamin, T. B. and Ellis, A. T.},
  journal = {Philosophical Transactions of the Royal Society of London A},
  volume  = {260},
  pages   = {221--240},
  year    = {1966},
  doi     = {10.1098/rsta.1966.0046},
}

@incollection{Delale,
  title     = {Bubble Dynamics and Shock Waves},
  editor    = {Delale, Can F.},
  series    = {Shock Waves Science and Technology Reference Library},
  volume    = {8},
  publisher = {Springer},
  address   = {Berlin, Heidelberg},
  pages     = {82},
  year      = {2013},
  note      = {Check whether a specific chapter author/title within this edited volume was intended},
}

@article{Plesset1971,
  title   = {Collapse of an initially spherical vapour cavity near a solid boundary},
  author  = {Plesset, M. S. and Chapman, R. B.},
  journal = {Journal of Fluid Mechanics},
  volume  = {47},
  pages   = {283--290},
  year    = {1971},
  doi     = {10.1017/S0022112071001058},
}

@article{Plesset1956,
  title   = {On the stability of the spherical shape of a vapor cavity in a liquid},
  author  = {Plesset, M. S. and Mitchell, T. P.},
  journal = {Quarterly of Applied Mathematics},
  volume  = {13},
  pages   = {419--430},
  year    = {1956},
  doi     = {10.1090/qam/79999},
}

@article{BlakeGibson1987,
  title   = {Cavitation bubbles near boundaries},
  author  = {Blake, J. R. and Gibson, D. C.},
  journal = {Annual Review of Fluid Mechanics},
  volume  = {19},
  pages   = {99--123},
  year    = {1987},
  doi     = {10.1146/annurev.fl.19.010187.000531},
}

@article{Robert2007,
  title   = {Cavitation bubble behavior inside a liquid jet},
  author  = {Robert, E. and Lettry, J. and Farhat, M. and Monkewitz, P. A. and Avellan, F.},
  journal = {Physics of Fluids},
  volume  = {19},
  pages   = {067106},
  year    = {2007},
  doi     = {10.1063/1.2738406},
}

@article{Gu2026,
  title   = {Cavitation--bubble interaction with an initially perturbed free surface},
  author  = {Gu, Jingyu and Liu, Zirui and Zhang, A-Man and Li, Shuai},
  journal = {Journal of Fluid Mechanics},
  volume  = {1034},
  pages   = {A3},
  year    = {2026},
}

@article{Phipps2010,
  title   = {Review: Laser-Ablation Propulsion},
  author  = {Phipps, C. R. and Birkan, M. and Bohn, W. and Eckel, H.-A. and Horisawa, H. and Lippert, T. and Michaelis, M. and Rezunkov, Y. and Sasoh, A. and Schall, W. and Scharring, S. and Sinko, J.},
  journal = {Journal of Propulsion and Power},
  volume  = {26},
  number  = {4},
  pages   = {609--637},
  year    = {2010},
  doi     = {10.2514/1.43733},
}

@article{science2025,
  title   = {Launching by cavitation},
  author  = {Wang, Dalei and Liu, Zixiao and Zhao, Hongping and Qin, Huanqi and Bai, Gongxun and Chen, Chi and Shi, Pengju and Du, Yingjie and Zhao, Yusen and Liu, Wei and Wang, Dan and Zhou, Guoquan and He, Ximin and Dai, Chaoqing},
  journal = {Science},
  volume  = {389},
  pages   = {935--939},
  year    = {2025},
  doi     = {10.1126/science.adu8943},
}

@article{Singh2026,
  title   = {Predicting and controlling laser-induced breakup and multidirectional propulsion of liquid droplets},
  author  = {Singh, Awanish Pratap and Rao, D. Chaitanya Kumar and Rahlves, Maik and Vogel, Alfred and Basu, Saptarshi},
  journal = {Proceedings of the National Academy of Sciences},
  volume  = {123},
  pages   = {e2526933123},
  year    = {2026},
  doi     = {10.1073/pnas.2526933123},
  note    = {Original bibliography entry omitted co-author Alfred Vogel; corrected here},
}

@article{Favre2002,
  title   = {White-light nanosource with directional emission},
  author  = {Favre, C. and Boutou, V. and Hill, S. C. and Zimmer, W. and Krenz, M. and Lambrecht, H. and Yu, J. and Chang, R. K. and Woeste, L. and Wolf, J.-P.},
  journal = {Physical Review Letters},
  volume  = {89},
  pages   = {035002},
  year    = {2002},
  doi     = {10.1103/PhysRevLett.89.035002},
}

@article{Lindinger2004,
  title   = {Time-resolved explosion dynamics of H$_2$O droplets induced by femtosecond laser pulses},
  author  = {Lindinger, A. and Hagen, J. and Socaciu, L. D. and Bernhardt, T. M. and W{\"o}ste, L. and Duft, D. and Leisner, T.},
  journal = {Applied Optics},
  volume  = {43},
  pages   = {5263--5269},
  year    = {2004},
  doi     = {10.1364/AO.43.005263},
}

@article{Stan2016,
  title   = {Liquid explosions induced by X-ray laser pulses},
  author  = {Stan, C. and Milathianaki, D. and Laksmono, H. and Sierra, M. and McQueen, J. and Messerschmidt, M. and Williams, G. J. and Kogiso, M. and Nilsson, A. and Barty, N. and Hodgson, K. O.},
  journal = {Nature Physics},
  volume  = {12},
  pages   = {966--971},
  year    = {2016},
  doi     = {10.1038/nphys3779},
}

@article{Grunbein2021,
  title   = {Effect of X-ray free-electron laser-induced shockwaves on haemoglobin microcrystals delivered in a liquid jet},
  author  = {Gr{\"u}nbein, M. L. and others},
  journal = {Nature Communications},
  volume  = {12},
  pages   = {1672},
  year    = {2021},
  doi     = {10.1038/s41467-021-21819-9},
}

@article{Liu2021,
  title   = {Optofluidic resonance of a transparent liquid jet excited by a continuous-wave laser},
  author  = {Liu, H. and Wang, Z. and Gao, L. and Huang, Y. and Tang, H. and Zhao, X. and Deng, W.},
  journal = {Physical Review Letters},
  volume  = {127},
  pages   = {234501},
  year    = {2021},
  doi     = {10.1103/PhysRevLett.127.234501},
}

@article{Zhao2021,
  title   = {Uniform breaking of liquid jets by modulated laser heating},
  author  = {Zhao, Y. and Wan, D. and Chen, X. and Chao, X. and Xu, H.},
  journal = {Physics of Fluids},
  volume  = {33},
  pages   = {044115},
  year    = {2021},
  doi     = {10.1063/5.0046445},
}

@article{Nahas1990,
  title   = {Instability of a liquid jet in surface-tension flows},
  author  = {Nahas, N. M. and Panton, R. L.},
  journal = {Journal of Fluids Engineering},
  volume  = {112},
  pages   = {296--301},
  year    = {1990},
  doi     = {10.1115/1.2909405},
}

@article{Mondal2015,
  title   = {Controlling local temperature in water using femtosecond optical tweezer},
  author  = {Mondal, D. and Goswami, D.},
  journal = {Biomedical Optics Express},
  volume  = {6},
  pages   = {3190--3196},
  year    = {2015},
  doi     = {10.1364/BOE.6.003190},
}

@article{Kuiper2004,
  title   = {Variable-focus liquid lens for miniature cameras},
  author  = {Kuiper, S. and Hendriks, B. H. W.},
  journal = {Applied Physics Letters},
  volume  = {85},
  number  = {7},
  pages   = {1128--1130},
  year    = {2004},
  doi     = {10.1063/1.1779954},
}

@article{Tian2022,
  title   = {Adaptive liquid lens with a tunable field of view},
  author  = {Tian, J.-Q. and Zhao, Z.-Z. and Li, L.},
  journal = {Optics Express},
  volume  = {30},
  number  = {22},
  pages   = {40991--41001},
  year    = {2022},
  doi     = {10.1364/OE.472634},
}

@article{Dong2006,
  title   = {Adaptive liquid microlenses activated by stimuli-responsive hydrogels},
  author  = {Dong, L. and Agarwal, A. K. and Beebe, D. J. and Jiang, H.},
  journal = {Nature},
  volume  = {442},
  pages   = {551--554},
  year    = {2006},
  doi     = {10.1038/nature05024},
}

@article{Lopez2008,
  title   = {Fast focusing using a pinned-contact oscillating liquid lens},
  author  = {L{\'o}pez, C. A. and Hirsa, A. H.},
  journal = {Nature Photonics},
  volume  = {2},
  number  = {10},
  pages   = {610--613},
  year    = {2008},
  doi     = {10.1038/nphoton.2008.198},
}

@article{Nguyen2010,
  title   = {Micro-optofluidic lenses: A review},
  author  = {Nguyen, N.-T.},
  journal = {Biomicrofluidics},
  volume  = {4},
  number  = {3},
  pages   = {031501},
  year    = {2010},
  doi     = {10.1063/1.3460919},
}

@article{Vincenti2019,
  title   = {Achieving Extreme Light Intensities using Optically Curved Relativistic Plasma Mirrors},
  author  = {Vincenti, H.},
  journal = {Physical Review Letters},
  volume  = {123},
  pages   = {105001},
  year    = {2019},
  doi     = {10.1103/PhysRevLett.123.105001},
}

@article{Vincenti2023,
  title   = {Plasma mirrors as a path to the Schwinger limit: theoretical and numerical developments},
  author  = {Vincenti, H. and Clark, T. and Fedeli, L. and others},
  journal = {European Physical Journal Special Topics},
  volume  = {232},
  pages   = {2303--2346},
  year    = {2023},
  doi     = {10.1140/epjs/s11734-023-00953-2},
}

@article{Mondal2024,
  title   = {Shaped liquid drops generate MeV temperature electron beams with millijoule class laser},
  author  = {Mondal, Angana and Sabui, Ratul and Tata, Sheroy and Trines, R. M. G. M. and Rahul, S. V. and Li, Feiyu and Sarkar, Soubhik and Trickey, William and Kumar, Rakesh Y. and Rajak, Debobrata and Pasley, John and Sheng, Zhengming and Jha, Jagannath and Anand, M. and Gopal, Ram and Robinson, A. P. L. and Krishnamurthy, M.},
  journal = {Communications Physics},
  volume  = {7},
  pages   = {85},
  year    = {2024},
  doi     = {10.1038/s42005-024-01550-8},
}

@book{deGennes2004,
  title     = {Capillarity and Wetting Phenomena: Drops, Bubbles, Pearls, Waves},
  author    = {de Gennes, P.-G. and Brochard-Wyart, F. and Qu{\'e}r{\'e}, D.},
  publisher = {Springer},
  address   = {New York},
  year      = {2004},
}

@book{Lin2003,
  title     = {Breakup of Liquid Sheets and Jets},
  author    = {Lin, S.-P.},
  publisher = {Cambridge University Press},
  address   = {Cambridge},
  year      = {2003},
}

@book{Hecht,
  title     = {Optics},
  author    = {Hecht, E.},
  edition   = {5th},
  publisher = {Pearson Education},
  address   = {Harlow, United Kingdom},
  year      = {2017},
}



@inproceedings{2024diffractio,
  title     = {Diffractio: an open-source library for diffraction and interference calculations},
  author    = {Sanchez-Brea, L. M. and Bernabeu, E. and Porras, J. A. and Villarrubia, V. P. and Elshorbagy, M. H. and Mu{\~n}oz, J. d. H. and Milla, F. J. T. and Alda, J.},
  booktitle = {Proc. Optics and Photonics for Advanced Dimensional Metrology III},
  pages     = {46},
  year      = {2024},
}

@article{Fabin2006,
  title   = {Fast-Fourier-transform based numerical integration method for the Rayleigh--Sommerfeld diffraction formula},
  author  = {Shen, F. and Wang, A.},
  journal = {Applied Optics},
  volume  = {45},
  pages   = {1102--1110},
  year    = {2006},
  doi     = {10.1364/AO.45.001102},
}

@article{Kennedy1995,
  title   = {A First-Order Model for Computation of Laser-Induced Breakdown Thresholds in Ocular and Aqueous Media. I. Theory},
  author  = {Kennedy, P. K.},
  journal = {IEEE Journal of Quantum Electronics},
  volume  = {31},
  number  = {12},
  pages   = {2241--2249},
  year    = {1995},
  doi     = {10.1109/3.477753},
}

@article{Vogel1996,
  title   = {Shock wave emission and cavitation bubble generation by picosecond and nanosecond optical breakdown in water},
  author  = {Vogel, A. and Busch, S. and Parlitz, U.},
  journal = {Journal of the Acoustical Society of America},
  volume  = {100},
  pages   = {148--165},
  year    = {1996},
  doi     = {10.1121/1.415878},
}

@book{Brennen1995,
  title     = {Cavitation and Bubble Dynamics},
  author    = {Brennen, C. E.},
  publisher = {Oxford University Press},
  address   = {New York},
  year      = {1995},
}

@article{Dietrich2008,
  title   = {Passage of a Bubble Through a Liquid--Liquid Interface},
  author  = {Dietrich, N. and Poncin, S. and Pheulpin, S. and Li, H.-Z.},
  journal = {AIChE Journal},
  volume  = {54},
  number  = {3},
  pages   = {594--600},
  year    = {2008},
  doi     = {10.1002/aic.11399},
}

@article{Feit1974,
  title   = {Effect of refraction on spot-size dependence of laser-induced breakdown},
  author  = {Feit, M. D. and Fleck, Jr., J. A.},
  journal = {Applied Physics Letters},
  volume  = {24},
  number  = {4},
  pages   = {169--172},
  year    = {1974},
  doi     = {10.1063/1.1655142},
}

@article{Couairon2007,
  title   = {Femtosecond filamentation in transparent media},
  author  = {Couairon, A. and Mysyrowicz, A.},
  journal = {Physics Reports},
  volume  = {441},
  pages   = {47--189},
  year    = {2007},
  doi     = {10.1016/j.physrep.2006.12.005},
}

@misc{Singh2026Caustic,
  title         = {Caustic-Driven Fluidic Microlenses for Enhanced Nonlinear and High-Energy-Density Physics},
  author        = {Singh, Sourabh and Harsha, S. Sree and Tamanna and Singh, Prashant Kumar},
  eprint        = {2606.20125},
  archivePrefix = {arXiv},
  primaryClass  = {physics.optics},
  year          = {2026},
}

@book{Lambert1760,
  title     = {Photometria},
  author    = {Lambert, J. H.},
  publisher = {Eberhard Klett},
  address   = {Augsburg},
  year      = {1760},
}

@article{Beer1852,
  title   = {Bestimmung der Absorption des roten Lichts in farbigen Fl{\"u}ssigkeiten},
  author  = {Beer, A.},
  journal = {Annalen der Physik und Chemie},
  volume  = {162},
  pages   = {78--88},
  year    = {1852},
}

@article{NotzBasaran2004,
  title   = {Dynamics and breakup of a contracting liquid filament},
  author  = {Notz, P. K. and Basaran, O. A.},
  journal = {Journal of Fluid Mechanics},
  volume  = {512},
  pages   = {223--256},
  year    = {2004},
  doi     = {10.1017/S0022112004009759},
}

@article{Driessen2013,
  title   = {Stability of viscous long liquid filaments},
  author  = {Driessen, T. and Jeurissen, R. and Wijshoff, H. and Toschi, F. and Lohse, D.},
  journal = {Physics of Fluids},
  volume  = {25},
  pages   = {062109},
  year    = {2013},
  doi     = {10.1063/1.4811849},
}

@article{CastrejonPita2012,
  title   = {Breakup of Liquid Filaments},
  author  = {Castrej{\'o}n-Pita, A. A. and Castrej{\'o}n-Pita, J. R. and Hutchings, I. M.},
  journal = {Physical Review Letters},
  volume  = {108},
  pages   = {074506},
  year    = {2012},
  doi     = {10.1103/PhysRevLett.108.074506},
}

@book{BornWolf1999,
  title     = {Principles of Optics: Electromagnetic Theory of Propagation, Interference and Diffraction of Light},
  author    = {Born, M. and Wolf, E.},
  edition   = {7th},
  publisher = {Cambridge University Press},
  year      = {1999},
}


@article{2024diffractio,
  title     = {Diffractio: an open-source library for diffraction and interference calculations},
  author    = {Sanchez-Brea, L. M. and Bernabeu, E. and Porras, J. A. and Villarrubia, V. P. and Elshorbagy, M. H. and Mu{\~n}oz, J. d. H. and Milla, F. J. T. and Alda, J.},
  booktitle = {Proc. Optics and Photonics for Advanced Dimensional Metrology III},
  pages     = {46},
  year      = {2024},
}

@article{Fabin2006,
  title   = {Fast-Fourier-transform based numerical integration method for the Rayleigh--Sommerfeld diffraction formula},
  author  = {Shen, F. and Wang, A.},
  journal = {Applied Optics},
  volume  = {45},
  pages   = {1102--1110},
  year    = {2006},
  doi     = {10.1364/AO.45.001102},
}







